MEMROC: Multi-Eye to Mobile RObot Calibration

This paper presents MEMROC (Multi-Eye to Mobile RObot Calibration), a novel motion-based calibration method that simplifies the process of accurately calibrating multiple cameras relative to a mobile robot's reference frame. MEMROC utilizes a known calibration pattern to facilitate accurate calibration with a lower number of images during the optimization process. Additionally, it leverages robust ground plane detection for comprehensive 6-DoF extrinsic calibration, overcoming a critical limitation of many existing methods that struggle to estimate the complete camera pose. The proposed method addresses the need for frequent recalibration in dynamic environments, where cameras may shift slightly or alter their positions due to daily usage, operational adjustments, or vibrations from mobile robot movements. MEMROC exhibits remarkable robustness to noisy odometry data, requiring minimal calibration input data. This combination makes it highly suitable for daily operations involving mobile robots. A comprehensive set of experiments on both synthetic and real data proves MEMROC's efficiency, surpassing existing state-of-the-art methods in terms of accuracy, robustness, and ease of use. To facilitate further research, we have made our code publicly available at https://github.com/davidea97/MEMROC.git.

==> tex/1_intro.tex <==
\begin{comment}
%
Spiegare importanza di calibrare uno o più sensori rispetto ad un robot mobile. Quali sono le possibili applicazioni? \\
Prendo spunti da SensorX2Car, R-AL, Opencalib\\
Introdurre il problema della z inosservabile.\\
Evidenziare e mettere in luce che maggior parte di lavori stimano solo 3DoF oppure trasformata tra sensori che però non risolve problema. \\
\textbf{Cosa faccio di nuovo?}
Claim: riusciamo a risolvere il problema della calibrazione con poche immagini (meno di 10)\\
Setup molto semplice (basta un pattern di calibrazione messo dove si vuole), non serve avere un ambiente controllato con molti landmarks o con traiettorie ben definite. Sia indoor che outdoor proprio perchè non richiedo particolari attrezzature e/o ambienti controllati.\\
Non ho vincoli sulle traiettorie (non devo fare cerchi, o pattern come l’8, guardare OpenCalib).\\

\textbf{Cosa propongo?}
Metodo basato su pattern e ground floor detection, per calibrare sensori RGB o RGB-D rispetto ad una frame di riferimento del robot\\
Tutti quelli che fanno ground floor detection si basano su ricostruzioni SoF e prendono la misura anche solo una volta, però dispendiosa perchè richiedono molte immagini. A me bastano poche immagini\\
Verifico la correttezza del piano trovato con RANSAC in modo tale che sia parallelo al vettore 0 0 1. Questo non è possibile se troviamo solo il piano rispetto alla telecamera ma è necessario ruotarlo rispetto al nostro world.\\ Entra in gioco la nostra SVD che è calcolata con le traiettorie.\\
Il pattern ci permette di superare anche il problema del fattore di scala che si ha senza usare il pattern\\
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% General intro, evidenziare perchè serve
Mobile robots require multiple sensors in order to perceive the environment and navigate autonomously within it.
The accurate alignment of visual and motion information enhances a mobile robot's perception, mapping, localization, and overall capability to interact effectively with its environment.
Fusaro \cite{fusaro2022pushing} proposes a traversability analysis for autonomous vehicles that combines geometric and appearance-based features, requiring precise camera calibration to translate visual information into the robot's reference frame for safe navigation. 
Even in Visual Odometry~\cite{nister2004visual, evangelidis2021revisiting}, to correctly estimate the robot motion from camera images, it is required knowing the spatial transformation between the camera and the reference frame of the mobile robot. Similarly, Zheng et al. \cite{zheng2019visual} address the localization and mapping problem for ground vehicles using odometry and monocular cameras. Their approach also necessitates the spatial transformation between the camera and the robot for accurate robot localization based on visual features. 
% Main challenges (3DOF)
% Sfida 1, servono setup molto particolari e costosi
The current prominent solution relies on accurate sensor installation in the factory in the first place or performs calibration in artificially-arranged rooms which contain specially-designed facilities such as markers-infrastructure \cite{xie2018infrastructure,antonelli2010simultaneous}, the usage of additional sensors~\cite{gao2010line}, manually calibrating cameras by moving a calibration pattern in front of the sensors~\cite{wang2022accurate}. 
%Although these methods can provide adequate precision, they are time-consuming and require expensive equipment, making it hard to realize in users’ hands. Unfortunately, due to the vibration and operating condition changes in daily use, the extrinsic parameter of sensors won’t stay the same. This calls for online target-free calibration methods.
While traditional calibration methods achieve good accuracy, they can be laborious and require specialized equipment, limiting their accessibility.  Furthermore, sensor performance can drift due to vibrations and varying operating conditions during everyday use. This necessitates a fast and user-friendly calibration technique for maintaining optimal sensor performance.
One significant challenge arises from the fact that the extrinsic parameters, particularly rotation, between the sensors and the vehicle can undergo changes due to daily vibrations and operating condition variations, rendering the initial calibration less effective in real-world scenarios. In response to these challenges, the focus is shifting towards online calibration methods that can adapt to dynamic conditions during the operational life of the vehicle.

% Sfida 2, non si riesce a stimare tutti gradi libertà perchè Z non osservabile
\textcolor{red}{However, most prior methods focus on extrinsic calibration between sensors, and few focus on the misalignment between the sensors and the vehicle coordinate system}


% Focus of the paper. What is proposed?
In this work, we investigate hand-eye based calibration methods to estimate the rototranslation between several cameras mounted on a mobile vehicle and the vehicle itself.
\textcolor{blue}{
In this paper, we explore the transition from traditional calibration methods to online approaches, focusing on the extrinsic calibration of cameras with respect to the odometry reference frame. We delve into the challenges posed by changes in extrinsic parameters during daily use and discuss the significance of aligning sensors with the vehicle for precise decision-making in autonomous driving scenarios. Additionally, we highlight the need for user-friendly and realizable calibration methods that can be applied seamlessly in diverse operational environments, marking a significant stride towards the practical implementation of autonomous vehicles in everyday scenarios.
}


% CLAIM
% - Stimo tutti 6 parametri estrinseci 
% - Servono poche immagini (+ veloce)
% - Più accurato dello stato arte
Summarizing, this paper present the following contributions:
(i) a camera-to-odometer calibration method which allows to accurately estimate the full set of 6 parameters describing the camera pose with respect to the wheels reference frame, generally assumed as vehichle reference frame;
(ii) Joint optimization in multi-camera system with overlapping field-of-view
(iiI) Dataset
(iv) an extensive evaluation of the proposed method in simulation and real indoor/outdoor scenarios, proving the robustness and precision of the calibration results.

==> tex/3_method_draft.tex <==
%To achieve robust and precise estimation of the whole six degrees of freedom (DoF) describing the sensor-to-robot transformation, we propose a two-step approach.  The first step involves ground plane estimation, addressing the inobservability of the z-coordinate (Section~\ref{subsec:ground_detection}).  The second step, detailed in Sections~\ref{subsec:overlap_calib} and~\ref{subsec:nonoverlap_calib}, performs optimization for 6 DoFs estimation, with separate procedures based on whether the sensors have overlapping fields of view.

Building upon the limitations identified in existing calibration methods, particularly the requirement for specific environmental conditions or limited DoF estimation, we propose a novel single-stage motion-based calibration process that incorporates a robust ground plane estimation as a preprocessing step (Section~\ref{subsec:ground_detection}). This estimated ground plane allows us to overcome the z-coordinate inobservability and achieve robust 6DoF calibration. The core calibration procedure adapts to the specific case of cameras with overlapping or non-overlapping fields of view (Sections~\ref{subsec:overlap_calib} and~\ref{subsec:nonoverlap_calib}). For overlapping fields of view, we propose a joint optimization approach that leverages the geometric relationships between the sensors to estimate all six degrees-of-freedom simultaneously.

TODO: SPIEGARE CHE PRENDIAMO LE MISURE DALLA SCACCHIERA 

\textcolor{red}{TODO: in questa overview del metodo manca una descrizione ad alto livello del metodo. Non viene mai detto ad esempio che è basato su hand-eye. Ci starebbe bene anche una schema a blocchi forse? 
}

\subsection{Ground plane detection}
\label{subsec:ground_detection}
%sezione plane detection (uso SVD per check sui piani “veri”) per avere valore z; caso RGB-D e RGB
Ground plane estimation is a critical preprocessing step for our calibration process. It allows us to overcome the z-coordinate inobservability inherent in 2D motion data. This section details our approach to robustly estimate the ground plane from sensor measurements. The method leverages the sensor's capabilities to obtain 3D points:
\begin{itemize}
\item RGBD Sensors: We directly utilize the rich 3D point cloud data provided by the sensor.
\item RGB Sensors: For sensors lacking depth information, we reconstruct 3D points by triangulating corresponding features between two consecutive frames by exploiting~\cite{morelli2022photogrammetry}. We exploit the relative transformation obtained through the motion based approach ($C_{t_{1}}$ to $C_{t_{2}}$) between these frames, which is efficiently obtained using the PnP algorithm~\cite{li2012robust} with the checkerboard pattern.
\end{itemize}

Once we have the 3D points, we identify the plane that best fits the majority of them using the RANSAC (RANdom SAmple Consensus) method. 
However, to ensure the identified plane truly represents the ground plane, we perform an additional refinement step.
%We leverage the Singular Value Decomposition (SVD) calculated during RANSAC. By analyzing the singular values obtained from SVD, we can further refine the plane parameters and achieve a more accurate representation of the ground surface.
%This two-pronged approach, combining RANSAC for initial estimation and SVD for refinement, ensures robust and reliable ground plane estimation, which is crucial for subsequent 6DoF calibration.


\subsection{Optimization Procedure for Multi-Sensor Calibration Without Overlapping}
\label{subsec:nonoverlap_calib}

Motion-based calibration of multiple sensors can be formulated as a hand-eye calibration problem, as illustrated in Figure X. This  formulation can be mathematically expressed as follow:

\begin{equation}
    A_{i}X = XB_{i},
\end{equation}

where $A_{i}$ and $B_{i}$ represent the robot's and sensor's motions, respectively, and $X$ is the transformation matrix we aim to estimate. Given N motion samples and M sensors on the robot, we minimize a cost function defined as:

\begin{equation}
    c_{k} = \sum_{i=0}^{N-1}\left[\left\|T_{R_{i}}^{R_{i+1}}T^{R}_{C} - T^{R}_{C}T_{C_{i}}^{C_{i+1}}\right\|_{2} + \left\|[T^{R}_{C}]_{z}-\overline{z_{i}}\right\|_{2}\right],
    \label{eq:minimization_eq}
\end{equation}

where $k\in[0,M]$. The first term minimizes the difference between consecutive relative poses of the robot and the sensor, ensuring their consistency. The second term minimizes the difference of the Z-coordinate in the sensor's translation vector $T^{R}_{C}$ with respect to the $i^{th}$ measurement provided by the ground detection $\overline{z_{i}}$.


\subsection{Joint Optimization procedure for multi-sensor with overlapping}
\label{subsec:overlap_calib}
In the case in which multiple sensors can simultaneously detect the checkerboard, we proposed a joint optimization between sensor which takes into account also the relative constraints existing among sensors, promising to more robust and accurate results even in presence of noisy odometry measurements.
The joint optimization aims to minimize also the following cost function:
\begin{equation}
    c_{cross} = 
\end{equation}

and
